Deep Stable Learning for Out-Of-Distribution Generalization

Approaches based on deep neural networks have achieved striking performance when testing data and training data share similar distribution, but can significantly fail otherwise. Therefore, eliminating the impact of distribution shifts between training and testing data is crucial for building performance-promising deep models. Conventional methods assume either the known heterogeneity of training data (e.g. domain labels) or the approximately equal capacities of different domains. In this paper, we consider a more challenging case where neither of the above assumptions holds. We propose to address this problem by removing the dependencies between features via learning weights for training samples, which helps deep models get rid of spurious correlations and, in turn, concentrate more on the true connection between discriminative features and labels. Extensive experiments clearly demonstrate the effectiveness of our method on multiple distribution generalization benchmarks compared with state-of-the-art counterparts. Through extensive experiments on distribution generalization benchmarks including PACS, VLCS, MNIST-M, and NICO, we show the effectiveness of our method compared with state-of-the-art counterparts.

==> paragraphs/intro_new.tex <==
\section{Introduction} \label{para:intro}

Many machine learning approaches tend to exploit subtle statistical correlations existing in the training distribution for predictions which have been shown to be effective under the I.I.D. hypothesis, i.e., testing and training data is independently sampled from the identical distribution.
In real cases, however, such a hypothesis can hardly be satisfied due to the complex generation mechanism of real data such as data selection biases, confounding factors, or other peculiarities.
The testing distribution may incur uncontrolled and unknown shifts from the training distribution, which makes most machine learning models fail to make trustworthy predictions \cite{arjovsky2019invariant, shen2020stable}.

\begin{figure}[th]
    \centering
    \includegraphics[width=\linewidth]{cvpr21/saliency_map_newfont.jpg}
    \caption{Visualization of saliency maps produced by the vanilla ResNet-18 model and our SWDG model when most of the training images containing dogs in the water.
    The lightness of the saliency map indicates how much attention that the models pay on particular area of the input image (i.e. lighter area plays a more crucial role for the prediction than the darker area).
    Due to the spurious correlation, the ResNet-18 model tends to focus on both dogs and the water while our model focuses mostly on dogs.}
    \label{fig:intro}
\end{figure}

% Key Factor
Essentially, when there incurs a distribution shift, the accuracy drop of current models is mainly caused by the spurious correlation between the irrelevant features (i.e. the features that are irrelevant to a given category, such as features of context, figure style, etc.) and category labels, and this kind of spurious correlations are intrinsically caused by the subtle correlations between irrelevant features and relevant features (i.e. the features that are relevant to a given category) \cite{lake2017building, marcus2018deep, lopez2017discovering, arjovsky2019invariant}. 
Taking the recognition task of `dog' category as an example, as depicted in Figure \ref{fig:intro}, if dogs are in the water in most training images, the visual features of dogs and water would be strongly correlated, thus leading to the spurious correlation between visual features of water with the label `dog'. 
As a result, when encountering images of dogs without water, or other objects (such as cats) with water, the model is prone to produce false predictions.

Recently, such distribution (domain) shift problems have been intensively studied in the \textsl{domain generalization (DG)} literature \cite{muandet2013domain,  ghifary2015domain,khosla2012undoing, wang2020learning,li2017deeper,li2019episodic}. 
The basic idea of DG is to divide a category into multiple domains so that irrelevant features vary across different domains while relevant features remain invariant \cite{khosla2012undoing, li2018domain, motiian2017unified}. 
Such training data makes it possible for a well-designed model to learn the invariant representations across domains and inhibit the negative effect from irrelevant features, leading to better generalization ability under distribution shifts. 
Some pioneering methods require clear and significant heterogeneity, namely that the domains are manually divided and labeled \cite{wang2017select, ganin2016domain, ratner2017learning, ding2017deep, niu2015multi}, which cannot be always satisfied in real applications. 
More recently, some methods are proposed to implicitly learn latent domains from data \cite{qiao2020learning, matsuura2020domain, wang2019learning}, but they implicitly assume that the latent domains are balanced, meaning that the training data is formed by balanced sampling from latent domains. 
In real cases, however, the assumption of domain balance can be easily violated, leading to the degeneration of these methods. 
This is also empirically validated in our experiments as shown in Section \ref{gen_inst}. 

Here we consider a more realistic and challenging setting, where the domains of training data are unknown and we do not implicitly assume that the latent domains are balanced. 
Given that the statistical dependence between relevant and irrelevant features is a major cause of model crash under distribution shifts, 
a straightforward approach is to decorrelate the relevant and irrelevant features. 
Since there is no extra supervision for separating relevant features from irrelevant features, a conservative solution is to decorrelate all features. 
Recently, this notion has been demonstrated to be effective in improving the generalization ability of linear models. 
\cite{kuang2020stable} proposes a sample weighting approach with the goal of decorrelating input variables, and \cite{shen2020stable} theoretically proves why such sample weighting can make a linear model produce stable predictions under distribution shifts.
But they are all developed under the constraints of linear frameworks.
When extending these ideas into deep models to tackle more complicated data types like images, we confront two main challenges. 
First, the complex non-linear dependencies among features are much more difficult to be measured and eliminated than the linear ones.
Second, the global sample weighting strategy in these methods requires excessive storage and computational cost in deep models, which is infeasible in practice.

To address these two challenges, we propose a method called \textbf{Sample Weighting for Distribution Generalization (SWDG)}.
In terms of the first challenge, we propose a novel nonlinear feature decorrelation approach based on Random Fourier Features \cite{rahimi2008random} with linear computational complexity. 
As for the second challenge, we propose an efficient optimization mechanism to perceive and remove correlations globally by iteratively saving and reloading features and weights of the model. 
These two modules are jointly optimized in our method. 
It should be noted that such a sample weighting method (i.e. SWDG) is actually a flexible plug-in module that can be integrated into any backbone models, such as ResNet \cite{he2016deep} or even existing DG methods. 
Our experimental results show that, after applying the sample weights learned by SWDG, ResNet can improve its classification accuracy by up to 7 percent under distribution shifts.
Moreover, as shown in Figure \ref{fig:intro}, SWDG can effectively partial our the irrelevant features (i.e. water) and leverage truly relevant features for prediction, which is more robust in the wild non-stationary environments.


